A Reparameterization-Invariant Flatness Measure for Deep Neural Networks

The performance of deep neural networks is often attributed to their automated, task-related feature construction. It remains an open question, though, why this leads to solutions with good generalization, even in cases where the number of parameters is larger than the number of samples. Back in the 90s, Hochreiter and Schmidhuber observed that flatness of the loss surface around a local minimum correlates with low generalization error. For several flatness measures, this correlation has been empirically validated. However, it has recently been shown that existing measures of flatness cannot theoretically be related to generalization due to a lack of invariance with respect to reparameterizations. We propose a natural modification of existing flatness measures that results in invariance to reparameterization.

==> functionIllustration.tex <==
\def\layersep{2.5cm}

\definecolor{input}{RGB}{56,54,80}
\definecolor{hidden}{RGB}{0,193,189}
\definecolor{output}{RGB}{179,132,184}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep, scale=0.6, transform shape]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=input];
    \tikzstyle{output neuron}=[neuron, fill=output];
    \tikzstyle{hidden neuron}=[neuron, fill=hidden];
    \tikzstyle{hidden neuron 2}=[neuron, fill=hidden];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron, pin=left:] (I-\name) at (0,-\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,5}
        \path[yshift=0.5cm]
            node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};
        
    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
    	\foreach \dest in {1,...,5}
    		\path (I-\source) edge (H1-\dest);    
            
    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,4}
    	\path[yshift=0.0cm]
	    	node[hidden neuron 2] (H2-\name) at (2.2*\layersep,-\y cm) {};

	% Connect every node in the input layer with every node in the
	% hidden layer.
	\foreach \source in {1,...,5}
		\foreach \dest in {1,...,4}
			\path[draw=black!50] (H1-\source) edge (H2-\dest);  

    % Draw the output layer node
    \node[output neuron,pin={[pin edge={->}]right:}, right of=H2-3] (O) at (2*\layersep,-2.5 cm) {};
    %\node[output neuron,pin={[pin edge={->}]right: $f = \psi\circ\phi$}, right of=H2-3] (O) at (2*\layersep,-2.5 cm) {};

    

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,4}
        \path (H2-\source) edge (O);

    % Annotate the layers
    \node[annot,node distance=1cm] (hl) at (4,0.6 cm) {hidden layers};
    \node[annot] at (0,0.6 cm) {input layer};
    \node[annot] at (7.5,0.6 cm) {output layer};
    
    
    %draw the curly brackets
    \draw [-,
    thick,
    decoration={
    	brace,
    	mirror,
    	raise=0.3cm,
    	amplitude=10pt
    },
    decorate
    ] (-0.5,-4.3) -- (3,-4.3) 
    node [pos=0.5,anchor=north,yshift=-1.3cm] {$\phi$}; 
    
    %draw the curly brackets
    \draw [-,
    thick,
    decoration={
    	brace,
    	mirror,
    	raise=0.3cm,
    	amplitude=10pt
    },
    decorate
    ] (3.5,-4.3) -- (8,-4.3) 
    node [pos=0.5,anchor=north,yshift=-1.3cm] {$\psi$}; 
\end{tikzpicture}

